Intra-domain and cross-domain transfer learning for time series data -- How transferable are the features?

In practice, it is very demanding and sometimes impossible to collect datasets of tagged data large enough to successfully train a machine learning model, and one possible solution to this problem is transfer learning. This study aims to assess how transferable are the features between different domains of time series data and under which conditions. The effects of transfer learning are observed in terms of predictive performance of the models and their convergence rate during training. In our experiment, we use reduced data sets of 1,500 and 9,000 data instances to mimic real world conditions. Using the same scaled-down datasets, we trained two sets of machine learning models: those that were trained with transfer learning and those that were trained from scratch. Four machine learning models were used for the experiment. Transfer of knowledge was performed within the same domain of application (seismology), as well as between mutually different domains of application (seismology, speech, medicine, finance). We observe the predictive performance of the models and the convergence rate during the training. In order to confirm the validity of the obtained results, we repeated the experiments seven times and applied statistical tests to confirm the significance of the results. The general conclusion of our study is that transfer learning is very likely to either increase or not negatively affect the predictive performance of the model or its convergence rate. The collected data is analysed in more details to determine which source and target domains are compatible for transfer of knowledge. We also analyse the effect of target dataset size and the selection of model and its hyperparameters on the effects of transfer learning.

==> performance.tex <==
\begin{table}[h]
\caption{Average percentual gain in predictive performance across seven reruns of the experiment.}
\begin{adjustwidth}{-1in}{-1in} % adjust the L and R margins by 1 inch
\hspace*{7em}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
  & \textbf{LOMAX 1k5} & \textbf{LOMAX 9k} & \textbf{LEN-DB 1k5} & \textbf{LEN-DB 9k} & \textbf{STEAD 1k5} & \textbf{STEAD 9k} & \textbf{SPEECH 1k5} & \textbf{SPEECH 9k} & \textbf{EMG 1k5} & \textbf{EMG 9k} & \textbf{S\&P 500 1k5} & \textbf{S\&P 500 9k}\\ \hline
ConvNetQuake INGV [LOMAX] & - & - & \cellcolor{green} 13.6\% (0.01796) & 0.226\% (0.7353) & \cellcolor{green} 5.63\% (0.01796) & \cellcolor{green} 3.16\% (0.01796) & \cellcolor{red} -29.6\% (0.02799) & \cellcolor{green} 7.95e+02\% (0.01796) & \cellcolor{green} 29.3\% (0.02799) & \cellcolor{green} 40.2\% (0.01796) & \cellcolor{green} 80.8\% (0.01796) & \cellcolor{green} 77.1\% (0.01796) \\ \hline
MagNet [LOMAX] & - & - & 2.59\% (0.2367) & 0.7\% (1.0) & 5.68\% (0.09097) & 4.31\% (0.3105) & \cellcolor{green} 28.1\% (0.04252) & \cellcolor{green} 1.62e+03\% (0.01796) & \cellcolor{green} 26.0\% (0.02799) & \cellcolor{green} 10.7\% (0.01796) & \cellcolor{green} 2.04\% (0.01796) & \cellcolor{green} 2.07\% (0.02799) \\ \hline
MLSTM FCN [LOMAX] & - & - & \cellcolor{green} 2.88\% (0.01796) & 1.24\% (0.3105) & \cellcolor{green} 5.65\% (0.01796) & \cellcolor{green} 1.36\% (0.01796) & \cellcolor{green} 81.3\% (0.01796) & 4.88\% (0.09097) & \cellcolor{green} 19.6\% (0.01796) & \cellcolor{green} 5.54\% (0.01796) & \cellcolor{green} 75.6\% (0.01796) & \cellcolor{green} 9.33\% (0.02799) \\ \hline
TCN [LOMAX] & - & - & \cellcolor{green} 13.7\% (0.02799) & \cellcolor{green} 10.5\% (0.01796) & \cellcolor{green} 9.58\% (0.02799) & \cellcolor{green} 7.03\% (0.01796) & \cellcolor{green} 1.03e+02\% (0.01796) & \cellcolor{green} 1.06e+03\% (0.01796) & \cellcolor{green} 21.8\% (0.01796) & \cellcolor{green} 13.8\% (0.01796) & \cellcolor{green} 23.2\% (0.01796) & \cellcolor{green} 2.75\% (0.01796) \\ \hline
ConvNetQuake INGV [LEN-DB] & 2.86\% (0.499) & 2.44\% (0.7353) & - & - & \cellcolor{green} 6.38\% (0.04252) & 0.684\% (0.1282) & \cellcolor{green} 7.62e+02\% (0.01796) & \cellcolor{green} 1.76e+03\% (0.01796) & \cellcolor{green} 25.0\% (0.02799) & \cellcolor{green} 29.5\% (0.02799) & \cellcolor{green} 81.2\% (0.01796) & \cellcolor{green} 76.5\% (0.01796) \\ \hline
MagNet [LEN-DB] & \cellcolor{green} 6.61\% (0.01796) & \cellcolor{green} 6.98\% (0.01796) & - & - & 3.07\% (0.09097) & \cellcolor{green} 2.1\% (0.01796) & \cellcolor{green} 2.75e+02\% (0.01796) & \cellcolor{green} 2.12e+03\% (0.01796) & \cellcolor{green} 28.7\% (0.02799) & \cellcolor{green} 12.5\% (0.01796) & 1.41\% (0.06298) & \cellcolor{green} 1.28\% (0.04252) \\ \hline
MLSTM FCN [LEN-DB] & \cellcolor{green} 7.19\% (0.01796) & \cellcolor{green} 2.55\% (0.01796) & - & - & \cellcolor{green} 5.69\% (0.01796) & \cellcolor{green} 0.863\% (0.04252) & \cellcolor{green} 67.2\% (0.01796) & -0.984\% (0.6121) & \cellcolor{green} 16.3\% (0.01796) & -0.759\% (0.499) & \cellcolor{green} 73.8\% (0.01796) & \cellcolor{green} 8.4\% (0.01796) \\ \hline
TCN [LEN-DB] & 16.3\% (0.06298) & 4.08\% (0.1763) & - & - & -5.18\% (0.06298) & \cellcolor{green} 6.42\% (0.01796) & \cellcolor{green} 1.32e+02\% (0.01796) & \cellcolor{green} 9.63e+02\% (0.01796) & \cellcolor{green} 17.7\% (0.01796) & \cellcolor{green} 7.4\% (0.01796) & \cellcolor{green} 21.2\% (0.01796) & 2.1\% (0.06298) \\ \hline
ConvNetQuake INGV [STEAD] & -20.0\% (0.1763) & -10.9\% (0.398) & -0.601\% (0.7353) & -8.65\% (0.2367) & - & - & \cellcolor{green} 8.59e+02\% (0.01796) & \cellcolor{green} 1.7e+03\% (0.01796) & \cellcolor{green} 25.5\% (0.01796) & \cellcolor{green} 29.5\% (0.02799) & \cellcolor{green} 81.7\% (0.01796) & \cellcolor{green} 76.4\% (0.01796) \\ \hline
MagNet [STEAD] & \cellcolor{green} 6.62\% (0.01796) & \cellcolor{green} 5.59\% (0.01796) & -0.112\% (0.8658) & 0.187\% (0.6121) & - & - & \cellcolor{green} 3.11e+02\% (0.01796) & \cellcolor{green} 2.12e+03\% (0.01796) & \cellcolor{green} 28.3\% (0.02799) & \cellcolor{green} 14.2\% (0.01796) & 1.35\% (0.06298) & \cellcolor{green} 1.63\% (0.04252) \\ \hline
MLSTM FCN [STEAD] & \cellcolor{green} 7.13\% (0.01796) & 1.75\% (0.09097) & \cellcolor{green} 3.09\% (0.01796) & -0.296\% (0.6121) & - & - & \cellcolor{green} 60.7\% (0.01796) & -2.75\% (0.09097) & \cellcolor{green} 13.9\% (0.01796) & -2.01\% (0.2367) & \cellcolor{green} 74.7\% (0.01796) & \cellcolor{green} 10.2\% (0.01796) \\ \hline
TCN [STEAD] & 10.9\% (0.09097) & -3.95\% (0.499) & -0.152\% (1.0) & \cellcolor{green} 6.7\% (0.01796) & - & - & \cellcolor{green} 61.6\% (0.01796) & \cellcolor{green} 5.05e+02\% (0.01796) & 7.01\% (0.06298) & -1.44\% (0.398) & \cellcolor{green} 19.6\% (0.01796) & \cellcolor{green} 2.39\% (0.01796) \\ \hline
ConvNetQuake INGV [SPEECH] & \cellcolor{green} 5.66\% (0.04252) & \cellcolor{green} 10.1\% (0.01796) & \cellcolor{green} 10.5\% (0.02799) & \cellcolor{green} 2.32\% (0.01796) & \cellcolor{red} -6.52\% (0.02799) & \cellcolor{green} 2.98\% (0.02799) & - & - & \cellcolor{green} 33.5\% (0.01796) & \cellcolor{green} 48.2\% (0.01796) & \cellcolor{green} 79.8\% (0.01796) & \cellcolor{green} 74.2\% (0.01796) \\ \hline
MagNet [SPEECH] & -1.09\% (0.7353) & 3.45\% (0.09097) & 0.919\% (0.7353) & -0.37\% (0.398) & -0.0623\% (1.0) & 0.575\% (0.8658) & - & - & \cellcolor{green} 6.91\% (0.02799) & -1.91\% (0.3105) & \cellcolor{green} 1.66\% (0.01796) & 1.0\% (0.2367) \\ \hline
MLSTM FCN [SPEECH] & \cellcolor{green} 5.14\% (0.02799) & 0.612\% (0.7353) & \cellcolor{green} 2.83\% (0.01796) & 0.481\% (0.7353) & -0.782\% (0.499) & -1.69\% (0.2367) & - & - & 3.76\% (0.3105) & -2.79\% (0.398) & \cellcolor{green} 74.5\% (0.01796) & \cellcolor{green} 9.58\% (0.01796) \\ \hline
TCN [SPEECH] & \cellcolor{green} 27.4\% (0.01796) & 0.202\% (0.499) & \cellcolor{green} 3.63\% (0.02799) & \cellcolor{green} 10.3\% (0.01796) & -1.86\% (0.2367) & -1.58\% (0.7353) & - & - & \cellcolor{green} 9.81\% (0.01796) & -3.97\% (0.06298) & \cellcolor{green} 20.3\% (0.01796) & \cellcolor{green} 1.5\% (0.04252) \\ \hline
ConvNetQuake INGV [EMG] & \cellcolor{green} 4.92\% (0.02799) & \cellcolor{green} 14.2\% (0.01796) & \cellcolor{green} 6.64\% (0.02799) & \cellcolor{green} 1.98\% (0.01796) & -2.1\% (0.398) & \cellcolor{green} 3.17\% (0.02799) & \cellcolor{green} 1.18e+03\% (0.01796) & \cellcolor{green} 4.07e+03\% (0.01796) & - & - & \cellcolor{green} 76.1\% (0.01796) & \cellcolor{green} 72.0\% (0.01796) \\ \hline
MagNet [EMG] & \cellcolor{green} 4.11\% (0.01796) & 1.71\% (0.398) & -2.29\% (0.3105) & -0.706\% (0.2367) & 2.84\% (0.3105) & \cellcolor{green} 2.2\% (0.02799) & \cellcolor{green} 1.04e+02\% (0.01796) & \cellcolor{green} 2.16e+03\% (0.01796) & - & - & 0.967\% (0.1282) & 0.92\% (0.3105) \\ \hline
MLSTM FCN [EMG] & \cellcolor{green} 6.69\% (0.01796) & \cellcolor{green} 2.33\% (0.01796) & \cellcolor{green} 2.86\% (0.01796) & \cellcolor{green} 1.92\% (0.04252) & \cellcolor{green} 6.29\% (0.01796) & \cellcolor{green} 1.51\% (0.01796) & \cellcolor{green} 89.5\% (0.01796) & \cellcolor{green} 6.55\% (0.04252) & - & - & \cellcolor{green} 69.2\% (0.01796) & -2.45\% (0.8658) \\ \hline
TCN [EMG] & \cellcolor{green} 20.8\% (0.01796) & 3.12\% (0.3105) & \cellcolor{red} -7.43\% (0.01796) & -1.57\% (0.499) & -2.44\% (0.06298) & 1.29\% (0.398) & \cellcolor{green} 96.6\% (0.01796) & \cellcolor{green} 1.04e+03\% (0.01796) & - & - & \cellcolor{green} 21.1\% (0.01796) & \cellcolor{green} 2.42\% (0.01796) \\ \hline
ConvNetQuake INGV [S\&P 500] & -14.0\% (0.2367) & 0.439\% (1.0) & 1.58\% (0.7353) & 1.37\% (0.2367) & -20.0\% (0.2367) & -5.24\% (0.2367) & \cellcolor{green} 2.61e+02\% (0.01796) & \cellcolor{green} 1.01e+03\% (0.01796) & \cellcolor{green} 34.1\% (0.01796) & \cellcolor{green} 39.8\% (0.01796) & - & - \\ \hline
MagNet [S\&P 500] & -8.96\% (0.1282) & -2.51\% (0.499) & -7.98\% (0.06298) & -0.912\% (0.2367) & 1.04\% (0.6121) & 0.504\% (0.8658) & \cellcolor{green} 65.7\% (0.02799) & \cellcolor{green} 1.75e+03\% (0.01796) & \cellcolor{green} 8.71\% (0.02799) & \cellcolor{green} 7.61\% (0.01796) & - & - \\ \hline
MLSTM FCN [S\&P 500] & \cellcolor{green} 3.61\% (0.04252) & 0.165\% (0.7353) & 1.49\% (0.1282) & 0.266\% (0.8658) & -2.13\% (0.2367) & -0.874\% (0.2367) & \cellcolor{green} 1.01e+02\% (0.01796) & \cellcolor{green} 9.84\% (0.01796) & 4.69\% (0.2367) & 0.467\% (0.8658) & - & - \\ \hline
TCN [S\&P 500] & \cellcolor{green} 19.8\% (0.04252) & 2.33\% (0.2367) & 1.22\% (0.1763) & \cellcolor{green} 3.81\% (0.04252) & \cellcolor{red} -7.88\% (0.04252) & -3.54\% (0.2367) & \cellcolor{green} 59.0\% (0.01796) & \cellcolor{green} 7.64e+02\% (0.01796) & \cellcolor{green} 13.1\% (0.01796) & -0.348\% (1.0) & - & - \\ \hline
\end{tabular}
\end{adjustwidth}
\end{table}


\begin{table}[h]
\caption{Average percentual gain in convergence rate across seven reruns of the experiment for the hyperparameters that achieved the best predictive performance.}
\begin{adjustwidth}{-1in}{-1in} % adjust the L and R margins by 1 inch
\hspace*{7em}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
  & \textbf{LOMAX 1k5} & \textbf{LOMAX 9k} & \textbf{LEN-DB 1k5} & \textbf{LEN-DB 9k} & \textbf{STEAD 1k5} & \textbf{STEAD 9k} & \textbf{SPEECH 1k5} & \textbf{SPEECH 9k} & \textbf{EMG 1k5} & \textbf{EMG 9k} & \textbf{S\&P 500 1k5} & \textbf{S\&P 500 9k}\\ \hline
ConvNetQuake INGV [LOMAX] & - & - & 9.61\%  (0.09097) & -7.56\%  (0.1763) & \cellcolor{green} 14.1\% (0.02799) & -1.92\%  (0.499) & -12.2\%  (0.1763) & -14.0\%  (0.06298) & 16.0\%  (0.06298) & 0.501\%  (0.6121) & \cellcolor{green} 5.3\% (0.02799) & 14.8\%  (0.1763) \\ \hline
MagNet [LOMAX] & - & - & 43.5\%  (0.2367) & -9.19\%  (0.499) & 32.6\%  (0.398) & 41.6\%  (0.1282) & 13.2\%  (0.1763) & -8.05\%  (0.499) & 12.3\%  (0.1282) & -0.491\%  (1.0) & \cellcolor{green} 5.35\% (0.01796) & \cellcolor{green} 3.06\% (0.01796) \\ \hline
MLSTM FCN [LOMAX] & - & - & \cellcolor{red} -5.98\% (0.01796) & -1.71\%  (0.6121) & -8.85\%  (0.1282) & 1.63\%  (0.8658) & 3.47\%  (0.2367) & \cellcolor{green} 5.94\% (0.01796) & 3.47\%  (0.398) & \cellcolor{red} -13.8\% (0.01796) & \cellcolor{green} 13.2\% (0.01796) & 1.4\%  (0.1763) \\ \hline
TCN [LOMAX] & - & - & -10.8\%  (0.1282) & 5.87\%  (0.2367) & 28.6\%  (0.09097) & 5.27\%  (0.6121) & -3.96\%  (0.2367) & \cellcolor{green} 34.4\% (0.01796) & \cellcolor{green} 21.3\% (0.02799) & 6.21\%  (0.06298) & 1.62\%  (0.8658) & 2.25\%  (0.2367) \\ \hline
ConvNetQuake INGV [LEN-DB] & 30.2\%  (0.06298) & 13.7\%  (0.2367) & - & - & 32.4\%  (0.2367) & -6.31\%  (1.0) & \cellcolor{green} 14.0\% (0.02799) & -4.24\%  (0.398) & -1.95\%  (0.6121) & -0.459\%  (0.8658) & \cellcolor{green} 3.8\% (0.01796) & 9.19\%  (0.7353) \\ \hline
MagNet [LEN-DB] & \cellcolor{green} 7.72\% (0.02799) & -0.0567\%  (0.398) & - & - & 0.901\%  (0.3105) & 21.6\%  (0.6121) & -1.33\%  (0.7353) & 6.05\%  (0.09097) & \cellcolor{green} 17.0\% (0.01796) & -5.45\%  (0.06298) & \cellcolor{green} 5.63\% (0.01796) & \cellcolor{green} 3.49\% (0.02799) \\ \hline
MLSTM FCN [LEN-DB] & 0.278\%  (0.499) & -3.84\%  (0.1282) & - & - & 5.71\%  (0.3105) & 3.38\%  (0.2367) & 5.65\%  (0.2367) & 4.76\%  (0.06298) & \cellcolor{green} 11.9\% (0.02799) & \cellcolor{red} -13.9\% (0.02799) & \cellcolor{green} 13.0\% (0.04252) & \cellcolor{green} 1.92\% (0.04252) \\ \hline
TCN [LEN-DB] & \cellcolor{green} 8.38\% (0.01796) & 17.1\%  (0.7353) & - & - & \cellcolor{green} 30.8\% (0.01796) & \cellcolor{green} 28.4\% (0.04252) & \cellcolor{red} -13.8\% (0.01796) & \cellcolor{green} 24.9\% (0.01796) & \cellcolor{green} 41.1\% (0.01796) & 5.18\%  (0.3105) & 3.3\%  (0.1282) & 0.0614\%  (0.7353) \\ \hline
ConvNetQuake INGV [STEAD] & 28.2\%  (0.3105) & 15.0\%  (0.09097) & \cellcolor{green} 57.4\% (0.01796) & 10.2\%  (0.6121) & - & - & \cellcolor{green} 17.1\% (0.01796) & 3.98\%  (1.0) & 2.91\%  (0.7353) & -9.11\%  (0.1282) & \cellcolor{green} 5.2\% (0.01796) & 30.3\%  (0.06298) \\ \hline
MagNet [STEAD] & \cellcolor{green} 26.4\% (0.01796) & -8.91\%  (0.1763) & 8.93\%  (0.499) & -4.69\%  (0.2367) & - & - & -11.9\%  (0.09097) & 2.33\%  (0.8658) & \cellcolor{green} 14.7\% (0.02799) & -5.3\%  (0.1282) & \cellcolor{green} 4.51\% (0.02799) & 2.15\%  (0.09097) \\ \hline
MLSTM FCN [STEAD] & -0.323\%  (0.8658) & -6.57\%  (0.06298) & -2.22\%  (0.398) & \cellcolor{red} -10.3\% (0.01796) & - & - & 5.28\%  (0.3105) & 1.98\%  (0.398) & \cellcolor{green} 17.9\% (0.02799) & \cellcolor{red} -18.1\% (0.01796) & \cellcolor{green} 12.6\% (0.02799) & \cellcolor{green} 1.92\% (0.01796) \\ \hline
TCN [STEAD] & \cellcolor{green} 11.9\% (0.01796) & 18.9\%  (0.7353) & \cellcolor{green} 26.3\% (0.01796) & \cellcolor{green} 35.1\% (0.01796) & - & - & -1.0\%  (0.8658) & 5.32\%  (0.3105) & \cellcolor{green} 33.6\% (0.01796) & 3.73\%  (0.3105) & \cellcolor{green} 2.32\% (0.04252) & \cellcolor{green} 4.46\% (0.02799) \\ \hline
ConvNetQuake INGV [SPEECH] & 18.7\%  (0.499) & 8.69\%  (0.7353) & 27.9\%  (0.8658) & 0.346\%  (0.3105) & 1.72\%  (0.1763) & \cellcolor{red} -6.38\% (0.04252) & - & - & \cellcolor{green} 16.6\% (0.02799) & 6.86\%  (0.6121) & \cellcolor{green} 2.93\% (0.02799) & 4.4\%  (1.0) \\ \hline
MagNet [SPEECH] & \cellcolor{green} 21.0\% (0.01796) & \cellcolor{red} -9.98\% (0.02799) & \cellcolor{red} -11.5\% (0.01796) & -2.2\%  (0.7353) & 4.7\%  (0.1763) & 2.55\%  (0.499) & - & - & 11.8\%  (0.06298) & \cellcolor{red} -5.93\% (0.04252) & \cellcolor{green} 5.75\% (0.01796) & \cellcolor{green} 2.61\% (0.01796) \\ \hline
MLSTM FCN [SPEECH] & -4.94\%  (0.1282) & -6.29\%  (0.2367) & -2.66\%  (0.1763) & \cellcolor{red} -8.39\% (0.01796) & \cellcolor{red} -5.73\% (0.01796) & 16.3\%  (0.8658) & - & - & 3.04\%  (0.8658) & \cellcolor{red} -15.7\% (0.02799) & \cellcolor{green} 14.2\% (0.01796) & \cellcolor{green} 1.46\% (0.04252) \\ \hline
TCN [SPEECH] & \cellcolor{green} 5.91\% (0.04252) & 20.3\%  (0.6121) & 8.03\%  (0.398) & 15.6\%  (0.2367) & 26.2\%  (0.1763) & 22.4\%  (0.398) & - & - & 24.0\%  (0.1763) & -5.66\%  (0.6121) & 1.63\%  (0.6121) & \cellcolor{green} 4.07\% (0.01796) \\ \hline
ConvNetQuake INGV [EMG] & 19.9\%  (0.7353) & 14.6\%  (0.06298) & 25.5\%  (0.2367) & -5.41\%  (0.3105) & \cellcolor{green} 28.3\% (0.01796) & 0.0097\%  (0.398) & 26.5\%  (0.1282) & 2.38\%  (0.499) & - & - & \cellcolor{green} 3.56\% (0.01796) & 26.5\%  (0.2367) \\ \hline
MagNet [EMG] & \cellcolor{green} 16.1\% (0.01796) & -13.1\%  (0.09097) & 21.0\%  (0.6121) & -2.71\%  (0.8658) & 15.9\%  (0.06298) & 37.3\%  (0.09097) & 4.45\%  (0.3105) & 6.91\%  (0.1282) & - & - & \cellcolor{green} 3.67\% (0.01796) & 2.18\%  (0.06298) \\ \hline
MLSTM FCN [EMG] & 1.11\%  (0.398) & -0.467\%  (0.8658) & -2.33\%  (0.06298) & \cellcolor{red} -8.68\% (0.04252) & \cellcolor{red} -6.81\% (0.01796) & \cellcolor{green} 9.81\% (0.04252) & 5.39\%  (0.3105) & 3.09\%  (0.1282) & - & - & \cellcolor{green} 13.7\% (0.01796) & 0.515\%  (0.2367) \\ \hline
TCN [EMG] & 3.45\%  (0.3105) & 22.1\%  (0.1282) & 15.2\%  (0.8658) & 15.6\%  (0.7353) & -1.47\%  (0.7353) & 4.17\%  (0.7353) & \cellcolor{red} -13.3\% (0.01796) & \cellcolor{green} 25.0\% (0.01796) & - & - & \cellcolor{green} 3.89\% (0.04252) & \cellcolor{green} 3.78\% (0.02799) \\ \hline
ConvNetQuake INGV [S\&P 500] & 12.0\%  (0.2367) & 13.6\%  (0.09097) & 35.0\%  (0.499) & 6.22\%  (0.8658) & 32.5\%  (0.2367) & 19.0\%  (0.2367) & 7.4\%  (0.3105) & -4.75\%  (0.398) & 1.62\%  (0.6121) & -0.0643\%  (0.8658) & - & - \\ \hline
MagNet [S\&P 500] & -2.88\%  (0.3105) & -8.59\%  (0.398) & 20.6\%  (0.398) & -8.83\%  (0.499) & 13.6\%  (0.2367) & 6.05\%  (0.1282) & 8.78\%  (0.1763) & 1.23\%  (0.8658) & 6.56\%  (0.499) & -4.52\%  (0.3105) & - & - \\ \hline
MLSTM FCN [S\&P 500] & -0.267\%  (0.3105) & -5.95\%  (0.1763) & -3.92\%  (0.09097) & \cellcolor{red} -8.61\% (0.01796) & \cellcolor{red} -5.88\% (0.04252) & 8.91\%  (0.3105) & 7.4\%  (0.2367) & 4.08\%  (0.3105) & 2.79\%  (0.398) & \cellcolor{red} -15.9\% (0.02799) & - & - \\ \hline
TCN [S\&P 500] & \cellcolor{green} 7.34\% (0.01796) & 18.2\%  (0.7353) & 3.44\%  (1.0) & 5.64\%  (0.2367) & -1.19\%  (0.398) & 21.6\%  (0.6121) & -4.4\%  (0.6121) & \cellcolor{green} 22.4\% (0.02799) & 21.5\%  (0.1282) & -3.84\%  (0.398) & - & - \\ \hline
\end{tabular}
\end{adjustwidth}
\end{table}
